A network analysis on cloud gaming: Stadia, GeForce Now and PSNow

Cloud gaming is a new class of services that promises to revolutionize the videogame market. It allows the user to play a videogame with basic equipment while using a remote server for the actual execution. The multimedia content is streamed through the network from the server to the user. This service requires low latency and a large bandwidth to work properly with low response time and high-definition video. Three of the leading tech companies, (Google, Sony and NVIDIA) entered this market with their own products, and others, like Microsoft and Amazon, are planning to launch their own platforms in the near future. However, these companies released so far little information about their cloud gaming operation and how they utilize the network. In this work, we study these new cloud gaming services from the network point of view. We collect more than 200 packet traces under different application settings and network conditions for 3 cloud gaming services, namely Stadia from Google, GeForce Now from NVIDIA and PS Now from Sony. We analyze the employed protocols and the workload they impose on the network. We find that GeForce Now and Stadia use the RTP protocol to stream the multimedia content, with the latter relying on the standard WebRTC APIs. They result in bandwidth-hungry and consume up to 45 Mbit/s, depending on the network and video quality. PS Now instead uses only undocumented protocols and never exceeds 13 Mbit/s.

==> 6_bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/didomenico.jpg}}]%
{Andrea Di Domenico} is a student attending master’s degree in Computer Engineering at Politecnico di Torino.  In  2020 he received the Bachelor's Degree in computer engineering from Politecnico di Torino, Italy, by attending the program for young talents. In spring 2020 he did an internship at SmartData@Polito research center for Big Data technologies. His Master's degree focuses on Artificial Intelligence and Data Analytics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/Gianluca_Perna_PhD.jpg}}]%
{Gianluca Perna} (S'20) is a PhD student at Politecnico di Torino and member of SmartData@Polito research center for Big Data technologies. He obtained a Bachelor's degree in Telecommunication engineering and a Master's degree in ICT For Smart Societies with an excellent grade, both in the same University. Thanks to his passion and expertise in Machine Learning, Internet of Things and Data analysis he obtained a six months research grant before starting his PhD in the SmartData group. He is also pursuing a patent in the field of Building Design and participating in an international project with the leading IT company Cisco.


\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/trevisan.jpg}}]{Martino Trevisan} (M'16)
received his PhD in 2019 from Politecnico di Torino, Italy.
He is currently an assistant professor (RTD-A) at the SmartData@Polito center in the same university.
He has been collaborating in both Industry and European projects and spent six months in Telecom ParisTech, France
working on High-Speed Traffic Monitoring during his M.Sc. He visited twice Cisco labs in San Jose in summer 2016 and 2017, as well as AT\&T labs during fall 2018.
His research interests are Big Data and Machine Learning applied to Network Measurements and Traffic Monitoring.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/luca.jpg}}]%
{Luca Vassio}(M'16) is currently an Assistant Professor with the Department of Electronics and Telecommunications, Politecnico di Torino, Italy. He received a Ph.D. 'cum laude' in telecommunication engineering in 2018 and a M.Sc.  degree in mathematical modeling for engineering in 2012. In the last years, he collaborated, among the others, with  UFMG, MIT, Bell Labs and GE Aviation. He is expert in creating analytical and data-driven models of real phenomena.  His research interests include many fields of data science, from big data analytics problems to the usage of statistics, machine learning and optimization approaches applied to internet measurements, mobility and human behaviour.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/giordano.png}}]%
{Danilo Giordano} (M'17)
Ph.D., is an Assistant Professor at Politecnico di Torino. He is member at the SmartData@Polito lab, working at the application of data science application to networks, smart cities and predictive maintenance problems. During 2014, he was a research intern at Narus Inc., studying network anomaly detection techniques. In 2016, he was a PhD visiting student at the CAIDA research center working on the implementation of a large scale system to collect and analyze BGP data. For this topic, he won the Applied Networking Research Prize by IETF. His broaden interests are in the fields of data analysis, big data, and networking.
\end{IEEEbiography}




==> makefile <==
DOC=0_main

all:
	pdflatex $(DOC)
	bibtex   $(DOC)
	pdflatex $(DOC)
	pdflatex $(DOC)

clean:
	find . -name '*~' -exec rm -f {} \;
	find . -name '*.aux' -exec rm -f {} \;
	rm -f texput.log $(DOC).log $(DOC).ps $(DOC).toc $(DOC).lo* $(DOC).bbl $(DOC).blg $(DOC).dvi $(DOC).out $(DOC).synctex.gz diff.bbl diff.blg

zip: ${sources} ${pdffiles}
	rm -f $(DOC).zip && zip -r $(DOC).zip *.tex *.bib *.bbl *.cls figures Makefile makefile

diff:
		latexdiff -c submission_version/latexdiff_conf.txt \
							--preamble=submission_version/latexdiff_preamble_old.tex \
		          --exclude-textcmd="subsection" \
	            --flatten submission_version/main.tex main.tex > diff.tex
		#pdflatex diff
		#bibtex diff
		pdflatex diff
		pdflatex diff

